A Large-scale Friend Suggestion Architecture

Online social as an extension of traditional life plays an important role in our daily lives. Users often seek out new friends that have significant similarities such as interests and habits, motivating us to exploit such online information to suggest friends to users. In this work, we focus on friend suggestion in online game platforms because in-game social quality significantly correlates with player engagement, determining game experience. Unlike a typical recommendation system that depends on item-user interactions, in our setting, user-user interactions do not depend on each other. Meanwhile, user preferences change rapidly due to fast changing game environment. There has been little work on designing friend suggestion when facing these difficulties, and for the first time we aim to tackle this in large scale online games. Motivated by the fast changing online game environment, we formulate this problem as friend ranking by modeling the evolution of similarity among users, exploiting the long-term and short-term feature of users in games. Our experiments on large-scale game datasets with several million users demonstrate that our proposed model achieves superior performance over other competing baselines.

==> backup/1_intro.tex <==
% \section{TODOs}
%  \todo{We need to conduct a sequential correlation analysis to tell them why we adopt attention but not RNN to model the similarity relations.}
 
%  \todo{To reduce the gap between user embedding and user's friend preference, we adopt... ps: to add a gate to reduce this gap (model need update)}

\section{Introduction }


With the rapid development of the World Wide Web, online is a new normality for people living in this era, in which common activities in our daily lives are heavily migrating to the Internet,
such as politics~\cite{AdamickKDD2005}, game~\cite{Zhang2017SIGIR}, social~\cite{Fisher2006,KwakWWW2010}. 
We often collect and analyze the online activities to improve our online experience. 
% One of the most successful practice is the recommendation systems~\cite{Tang2013Socialrecommendation} that analyzes the users' behaviors, such as viewing and purchasing, and then recommends items to users to fit the obtained profiles of individual users.
A popular practice is recommender systems~\cite{Tang2013Socialrecommendation}, which analyze user behavior like viewing and purchasing, and then recommend the items to users so as to fit the obtained profiles of the individual users. 
Apart from the need of items, we human have a natural desire to make friends because  friendship constitutes a critical part of humanity.
In recent years, the development of recommendation systems is mostly concentrated in a user-item setting~\cite{BOBADILLA20131}, however, recommending strangers to make friends is also a desirable feature in many applications like players in games and dating applications. 
%  particular in the case that users are anonymous, 
\emph{How can we suggest strangers to users in an online setting when their interactions are scarce, mostly unavailable in reality?} In this work, we aim at applying it to online games and refer to this setting as friend suggestion~\cite{Maayankdd2010,EpastoVLDB2015}. 

% However, prior efforts rarely considers this situation and focuses on the cases where sufficient interactions are available, such as %location-based mobile~\cite{Chu2013}, 
% %web information~\cite{ADAMIC2003},
% mutual social influence~\cite{Zheng2017FriendRI}, 
% scholar interaction~\cite{XU2019} and others~\cite{LI2020}.
% To distinguish the problem just described, we refer our task as \emph{friend suggestion}~\cite{Maayankdd2010,EpastoVLDB2015} that recommending strangers to users without noticeable interactions. 


% This setting makes the solutions from 
%traditional e-commerce recommendations or news recommendations often not applicable because these recommendation methods also depend on interactions.

% This is also significantly different from traditional e-commerce recommendations or news recommendations, in a large number of social apps and game apps, a user’s friendship behavior is sparse and random, which is not suitable for modeling user's friend interests via user's interaction sequence with strangers.
% In these scenario, the user’s interaction with the app and activity in the app is very rich even if it has less relation with user's friend preference.
% Thus, how to utilize these behavior to conduct friend recommendation is vital and difficult.



%  \textcolor{red}{Different to traditional e-commerce recommendations or news recommendations, in a large number of social apps and game apps, a user’s friendship behavior is sparse and random, which is not suitable for modeling user's friend interests via user's interaction sequence with strangers.
% In these scenario, the user’s interaction with the app and activity in the app is very rich even if it has less relation with user's friend preference.
% Thus, how to utilize these behavior to conduct friend recommendation is vital and difficult.}\todo{no sure about this }
% \emph{How can we match two strangers in dynamic online networks which share both membership and periodic temporal behavior?
% }


% While little effort has been made to study this subject in the literature~\cite{ADAMIC2003}. 





From the theory of homophily in sociology~\cite{McPherson2001}, we know that people tend to associate with people that have similar behaviors to each other, and people that we friend with tend to behave like each other over time. This motivates us that the key for the friend suggestion task is to find people that are similar to each other, and therefore we need to address the problem of estimating the similarity between users.
To be able to estimate similarity, information about user profiles~\cite{Raadprofile2010,Peled2013} and behaviors~\cite{Liu2012,Chen2014,Nguyen2018} has to be taken into account. 
It provides two different perspectives to model user preferences on decision making, including long-term and short-term intents. 
Users from online games generate abundant data consisting of both perspectives. 
Specifically, individual game players generate rich online activities from time to time, and many of them are collected in a sequential order that reflects user dynamics, capturing users' short-term changes.
By contrast, players' profiles provide a long-term perspective to describe players, since these contain slow change or fixed information such as gender and age, which often have a predominant influence on players' decisions. 
By fusing long-term and short-term information, we can obtain a more comprehensive representation of users and build a model on top of it to learn the similarity between users. 

% \textcolor{blue}{Existing works~\cite{} often treat these types of information separately by simply concatenating them. This may..
% }


% However, aforementioned works often treat the similarity as a static status, neglecting the evolution of similarity in time. Such an evolution is particularly important at games that players have different preferences at different times due to the fast-changing environments, such as playing modes, scenes, players' tiers. 

% To overcome this, we integrate the the evolution of similarity of players while modelling their profiles and activities through a proposed time-aware multi-view similarity scheme.






% Therefore, we need to capture these evolution by modelling their recently generated information.
% Generally speaking, users generate two major different types of information in the web, including slow changing information like profiles, and fast changing dynamics like players' actions at the game.

% As a contrast, we know that users often have stable preferences in the user-item recommendation systems, therefore, these 

% because uses' often show robust preference to certain items. Therefore, 
% Different to users' preferences in the user-item recommendation systems, 










%\todo{consider static features later, see if any improvement}

% In this paper, we focus on these time dependent sequences of users for the friend recommendation. 
% among different interactions in a session as well as the correlation of behavior patterns among different sessions, traditional sequential recommender systems are particularly interested in employing appropriate and effective machine learning (ML) approaches to model sequential data, 
% Sociologists call this phenomenon of being affected by one's friends "homophily" -- the tendency to associate with people similar to you and the people you associate with tend to act like you over time 
% Recommendation system ~\cite{Tang2013Socialrecommendation} is the most successful practice of data mining and machine learning in the real-world application, which is as a desire feature in many scenarios, such as social networks~\cite{}, video games~\cite{}, e-commerce~\cite{}.
% Typical recommendation systems act in the context of recommending items to users, which have been comprehensively analyzed in the past decade~\cite{}. 


% why relate work fail to do so
%Regarding the sequence features, 


%some confounding variables can be properties of neighbors in the friendship network.


% Existing friend recommendation 
% often relies on interaction messages between users, such as location-based mobile~\cite{Chu2013}, web information~\cite{ADAMIC2003}, mutual social influence~\cite{Zheng2017FriendRI}, scholar interaction~\cite{XU2019} and ~\cite{LI2020}.
% This setting is different to a more general case where interaction information is not accessible.

%  \textcolor{red}{Different to traditional e-commerce recommendations or news recommendations, in a large number of social apps and game apps, a user’s friendship behavior is sparse and random, which is not suitable for modeling user's friend interests via user's interaction sequence with strangers.
% In these scenario, the user’s interaction with the app and activity in the app is very rich even if it has less relation with user's friend preference.
% Thus, how to utilize these behavior to conduct friend recommendation is vital and difficult.}\todo{no sure about this }
% \emph{How can we match two strangers in dynamic online networks which share both membership and periodic temporal behavior?
% }

One popular way to exploit the aforementioned short-term and long-term features is by sequential recommendation~\cite{Chen2019BehaviorST} from traditional e-commerce recommendation settings, leveraging sequences of viewing or purchasing items in online shopping platforms. 
One may argue that we can collect user-user interaction sequences and apply existing sequential recommendation models~\cite{Quadrana2018survey, Chen2019kdd,2017Deep,2019Deep}. 
However, common online websites or mobile apps are not designed for the friend suggestion task, therefore, the direct interaction behavior of users is often sparse and random. 
In fact, interactions among users has significant difference to that of user-item setting.
On one hand, a user-item interaction sequence has consecutive dependencies over each other, reflecting a user's sequential decisions~\cite{ji2019sequential, wang2019sequential}.
Although user-user interactions happened in a sequential manner, 
the consecutive interactions are not necessary depending on each other as those in a user-item interaction sequence, suggesting that
we can not simply treat them as a logical sequence and use these existing sequential recommendation models to address our problem.
On the other hand, a user's preference over items is slow changing because a user’s general taste is often static with no or slow change over time~\cite{yakhchi2021learning}.  
While this may not hold for players in games because of the fast updating environment in games.
Unlike a real-world human that takes years to develop his/her taste, the player's role in the game changes rapidly to adapt to the surrounding, making his/her preferences about decision changes rather than static. To this end, the question then arises: how can we deal with friend suggestion without interactions and users' preferences are changing quickly? 




% \todo{missing sth here. To tackle this, we introduce the evolution of similarity of players while modelling their profiles and activities through a proposed time-aware multi-view similarity scheme.
% }


% Unlike a sequence of viewing an item or making a purchase on a website that is a reflection of a user's sequential decisions~\cite{ji2019sequential},  
% where each of them depends on previous ones. Therefore, we can model users' behaviors from their historical records and predict their next decision in a sequence. 

% However, interactions between users are fundamentally different from the user-item sequential interactions, where each user-user interaction tends to be a unique decision under a certain case.

%, therefore, these interactions are generated in the same manner, 
% Although these interactions happened in a sequential manner, 
% the consecutive interactions are not necessary depending on each other, suggesting that
% we can not simply treat them as a logical sequence and use these existing sequential recommendation models to address our problem.

% \todo{User's preference are less likely to change in , while the interests of making friends are change fast;. so we need to model the evolution.}



% \textcolor{red}{ \todo{ add this para ?} Different to traditional e-commerce recommendations or news recommendations, in a large number of social apps and game apps, a user’s friendship behavior is sparse and random, which is not suitable for modeling user's friend interests via user's interaction sequence with strangers.
% In these scenario, the user’s interaction with the app and activity in the app is very rich even if it has less relation with user's friend preference.
% Thus, how to utilize these behavior to conduct friend recommendation is vital and difficult.}\todo{no sure about this }



% Existing friend recommendation often relies on interaction messages between users, such as  location-based mobile~\cite{Chu2013}, web information~\cite{ADAMIC2003}, mutual social
% influence~\cite{Zheng2017FriendRI}, scholar interaction~\cite{XU2019} and ~\cite{LI2020}.

\begin{figure}[t]
    \footnotesize
    \centering
    \includegraphics[trim={0cm 9cm 3cm 1cm},clip,width=0.47\textwidth]{images/overview.pdf} \vsa\vsb
    \caption{ \footnotesize
    TTTT }
    \label{fig:overview}
\end{figure}

% Apart from the features selection, how to effectively quantize the similarity based on users' features is another key question of friend suggestion.



% \todo{this para may not needed here ?}
% Apart from the features selection, how to effectively quantize the similarity based on users' features is another key question of friend suggestion.
% The most commonly used similarity measurement is to compute the dot product~\cite{he2017ncf}or use multilayer perceptron (MLP)~\cite{RendleKZA20}.
% %, which are linear and nonlinear, respectively.  
% However, these may suffer from two issues: i) single perspective and ii) low interpretability.  Firstly, both measurements compute the similarity between users from one perspective. 
% We question the effectiveness of using a single metric to measure the similarity, especially for online user real-world data that exhibits complex feature variations due to sparsity, incompleteness, noisy~\cite{GARCIALOZANO2020}. 
% Also, people make friends for different reasons, for example, books, sports, movies, food, and others. Therefore, the similarity of the same pair of users may be different when viewing from different perspectives. 
% \textcolor{red}{Secondly, MLP provides a learned similarity measurement and aims to replace dot product by concatenating two embeddings, however, the integration of MLP is treated as a heuristic process to replace the dot product, making the proposed model lacks interpretability.}
% To address these issues, we propose the multiview similarity
% learning by generalizing the inner product
% with a set of parametric metrics, and provide a simple implementation through an MLP. 



To address the aforementioned issue, we propose a novel end-to-end solution that leverages user behavior evolution with the proposed similarity evolution modeling, called deep similarity evolutionary neural network ~(\ourmeth). 
Specifically, we first learn a low-dimensional embedding from user features at each time point by applying Gated Recurrent Units~\cite{chung2014empirical}, fusing the long-term information and the short-term information as the unified embedding. 
We then characterize the similarity between users over time by computing they similarity through an efficient generalized dot product model.
Next, we model the evolution of user preference over time using the obtained similarity along the time line implicitly, which is formalized by self-attention~\cite{vaswani2017attention}, with the goal of inferring the current preference from the past. 

% Next, we score the similarity between the obtained user embedding from multiple views with learnable parameters at different time points. 
% We then apply self-attention mechanism to extract attention scores to determine the closeness between users, which takes advantage of Transformer~\cite{vaswani2017attention}  to capture temporal dependency. 

% The core of our method is to define a multi-view scoring function for measuring the similarity between users' sequences that capturing the dynamics of similarities. 


To sum up, we have the following contributions:\\
% 1, We show how to define the problem
% of friend suggestion in the context of no user interaction.
% This is also the first work exploring friend suggestion by considering long-term and short-term information 
1, \textbf{Novelty.} We develop a novel end-to-end friend suggestion model by integrating both long-term and short-term information. 
To the best of our knowledge, this can be the first work on this task without relying on interactions among users, and also the first application to online game scenarios. \\
2, \textbf{Efficiency.} We evaluate our model on large scale data generated from a popular online game with millions of users, and show superior results over competing methods. 
3,\textbf{}


% 3,\textbf{Efficiency.}


% We have witnessed great success of using deep neural networks for recommendation systems~\cite{}.

% This would lead to a poor generalization ability~\cite{} due to overfitting in the training stage.

% generalizing the inner product
% with a parametric bilinear matrix 

% We have witnessed great success of using deep neural networks for recommendation systems~\cite{}.



% The key of our task is to measure the similarity between users effectively, i.e. the similarity of two individual users' sequences.  

% We know that people have different reasons to make friends with certain people, and these reasons changes along the time as well. Therefore, we need to measure similarity between users from multiple perspectives.


% Unlike the user-item sequence used in  clickstream recommendation systems~\cite{Quadrana2018survey, Chen2019kdd,2017Deep,2019Deep}, our scenario measures similarity between users depend on individual users' sequences.
% While the user-user interaction sequence, such as the friend application, has a major difference to the aforementioned user-item sequence because this type of sequence task driven sequence and 




% Additionally, the number of users are often over millions in popular apps, therefore, we can not apply models in pure academic environments due to the memory and computational cost, for example, graph signal process~\cite{} based models calculate the similarity of all pairs. 


% But individual users often generate plenty data in a sequence manner, such as actions in a game.

% more importantly this is not for the friend recommendation purpose.



% \todo{the definition of sequence, what and how }






% Our task falls into the general recommendation domain in general, and we have witnessed great success of using deep neural networks for recommendation systems~\cite{}. The main paradigm of recommendation systems now is to combine the embedding framework and the Multilayer Perceptron (MLP) network. 
% Briefly, researchers use an embedding methods, such as attention~\cite{}, to obtain a low dimensional representation and fed it into a MLP for classification. 
% Numerous embedding methods are proposed~\cite{}, but the computing of similarity for embedded features gets very little attention, often using a dot product directly. 
% The similarity measurement and embedding are two different ways to address the same issue of representation learning~\cite{} from implicit and explicit views, respectively. Therefore, the success of them should be mutually benefited, which can improve the downstream applications, like the classification in recommendation systems. While little work has been done to integrate the power of similarity learning into this paradigm.  Methods like~\cite{he2017ncf,} try to change this by using MLP to replace dot product, but they simply treat this as a heuristic process, making the proposed model less interpretable.

% Besides, research shows that measuring similarity from one perspective may not reliable when features are complicated, leading to a poor generalization ability~\cite{}. We will address these two problems together in our paper by incorporating a general similarity learning component into the model.




% which often relies on pre-defined similarity function and measure similarity from single perspective, i.e. dot product~\cite{}. Inevitably, this ignores the underlying relation between input embedding, assuming that dot product can capture sufficient relations in the features.
 






% In this paper we propose new framework to deal with the friend recommendation using users' activity sequence.

% In addition to these theoretical contributions, our work also includes a major algorithmic and experimental component. 

%Briefly, researchers use an embedding solution to obtain a low dimensional representation of users and fed it into an MLP to compute similarity among users.
% Some methodologies have realized the importance of the social network while doing user-item recommendation, treating social connection as an side information to enhance the embedding power~\cite{}.But this assumes the social network is known or partially observed. In general, models under this setting can not address our concerns directly because we need consider two stranger users at a time.
 




%, and the current research investigated the reasons that motivate people to make friends.

% We now heavily rely on online information to make decisions. 
% Inevitably, we practice our daily social activities online,


% Of particular interests, we focus on the problem of match 

% building a online social network is a fundamental necessity of most people, which is the corner stone of our society.
% One immediate question is how to match
% strangers to friends
% pair two strangers as friends online from the  perspective of websites, aiming to improving users' online experience.  

%  Maya Angelou, “a friend may be waiting behind a stranger’s face.




% Recommendation system ~\cite{Tang2013Socialrecommendation} is the most successful practice of data mining and machine learning in the real-world application, which is as a desire feature in many scenarios, such as social networks~\cite{}, video games~\cite{}, e-commerce~\cite{}.
% It often analyze the users' behaviors~\cite{}, such as viewing and purchasing, and then recommend items to users to fit the obtained profiles of individual users.
% The most common setting of such systems is about user-item recommendation,.
% More than the user-item iteration, users have rich information about user-user interconnection, 






% We focus on the friend recommendation task when giving each individual user's online activities

% under the setting that we can observe the each user's  online activity and aim to pair two strangers as friends.

% In this setting, the primary challenge


% are tall, relatively dense, and resident in a single machine’s memory.

% \emph{
% How can we pair users when observing their dynamic activities?
% }


% This technique provides an efficient way for users to interconnect with other online individuals, enabling a host of applications including chatting, teaming up to play, and group buying. 





% The gene  of social  is now well embedded in the general recommendation system, often called as social recommendation system~\cite{}, aiming to enhance the recommendation ability using the friend network. While this setting assumes the social friends are known or partially observed beforehand~\cite{}.




% \par
% \todo{we need to define what is positive labels before cite it}
% \textcolor{red}{Compared to a general item recommendation scenario, there are two main limitations in the friend recommendation system which %cause the restricted researches in recent years.
% have limited research til now.
% Firstly, the interaction data in the social network is often sparse~\cite{}, making the positive labels is difficult to collect.} 

% \textcolor{blue}{Secondly, commonly used similarity functions in recommendation systems are often pre-defined, such as dot product~\cite{}. Inevitably, this ignores the underlying relation between input embedding, assuming that dot product can capture sufficient relations in the features.

% current user-item similarity 


% item is a static object 
%  }
% Secondly, due to the...,  the traditional similarity modeling such as vector dot product can not be directed applied to calculate the preference score between user-pairs.  


% \par

% Though effective, aforementioned paradigm is i) restricted to a single perspective similarity measurement and ii) unrelated to labels in the recommendation.



% what the challenges and how existing work handle it

% what can we do?


==> backup/4_method.tex <==
% \begin{table}[!t]
% \centering
% %\scriptsize
% \begin{tabular}{ |l|c|c|}
%  \hline
% $\mathbf{X}$ &   \\
%  \hline
% $\mathbf{H}$  &    \\
%  \hline
% $\mathbf{C}$  &    \\
%   \hline
% $\mathbf{r}$  &    \\
%   \hline  
% $\mathbf{u}$  &    \\
%   \hline  
%  $\mathbf{Q}$  &    \\
%   \hline  
%   $\mathbf{K}$  &    \\
%   \hline  
% $W$  &   similarity matrix \\
%   \hline  
%  $\odot $ & The Hadamard product  \\
%   \hline
% \end {tabular}
% \caption{ Key notation used throughout the paper \todo{add all major symbols}}
% \label{table:notation}
% \end{table}

\begin{figure*}[t]
    \centering
    \small
    \captionsetup{font={small}}
    \setlength{\abovecaptionskip}{0pt}
    \setlength{\belowcaptionskip}{2pt}
	\includegraphics[scale=0.25]{images/dsen.pdf}
	\caption{The overall architecture of \ourmeth. \todo{too large, refer to paper  NCF fig3}}
    \label{DMGAN} 
\end{figure*} ~\label{fig:framework}



% \todo{rui: double check this part:}
% \textcolor{red}{The sequences' embedding is unique but not independent, each  i think it can not be trained in a parallel style  }
% Note that sequences' embedding is independent to each other, therefore, we can do a parallel style training through a distributed system.  This is particularly attractive for large scale datasets, where popular applications often have millions users.
% \todo{next,we need to tell how to do the inference.}




% A notable property of our architecture is that, while our model is trained end-to-end, the item embedding computation is independent for each item. Since most of the computation is done during item embedding, we can pre-compute such embeddings in an offline process. Then, during inference, we fetch relevant item embeddings and only compute the buyer and context embeddings on- the-fly. This is particularly attractive in a production environment, since inference can be done efficiently online without compromising on up-to-date buyer purchase histories.

\section{Deep Neural Friend suggestion }






\subsection{Problem Formulation }
% In this section we first introduce the definition of friend suggestion and then introduce the 

We now present the problem of friend suggestion, defining as follows:
Given a pair of users $\left ( u_a,u_b \right )$, our goal is to determine their closeness through a model as $\mathcal{F}\left ( u_a,u_b \right )$.
% Given users' fast changing and slow changing information,
% % , that user $i$  has a sequence as $S_i=\left [ x_1,...,x_t \right ] $ 
% our goal is to determine the closeness of any given pair users, $\left ( u_a,u_b \right )$, through a model as $\mathcal{F}\left ( u_a,u_b \right )$.
For a given online platform, an individual user $i$ has both long-term information and short-term information, denoting as $R_i$ and $S_i$, respectively. The short-term information is from the user's instant online activities. For players in a game,
this contains their actions in a game, such as battles, moving traces and so on. Formally, these can be represented as sequences that collecting from $t$ time slots: $S_i=\left [ x_1,...,x_t \right ]$, %providing a refined granularity to
capturing the evolution of users' actions over time. 
While  long-term information often includes features that changing is slow or constant over a long period, such as profiles.  We integrate these two types of features to describe a user
while maintaining  time sensitivity.
In particular, we know little about the social relations between users, and the interactions between users are often sparse in our setting, which is often the case of suggesting strangers to users.
This setting is rarely considered in the literature, therefore existing solutions are often not applicable to this case. 
This work aims to address the problem of friend suggestion to users by employing the aforementioned features.


% \todo{why not using usr_id; special case in games privacy. }


% In this work we focus on the game platform, we extract users' dynamic activities as short-term features and profiles as long-term features. More specifically, we use users' daily actions in a game

% More specifically, the slow changing information of user-$i$ is denoting as  $R_i=\left [r_1,...,r_j \right ] $, and the fast changing information is denoted as a sequence of $S_i=\left [ x_1,...,x_t \right ] $ that collecting from $t$ time slots.



% With the aforementioned features, 
% we aim to learn a model $\mathcal{F}$ through a multiple-stage deep structure to implement this friend suggestion by ranking people in the candidate set.
% %, underlining the time dependency and multiple perspectives of sequence data of online users. 
% A overview of our model is shown in the Figure ~\ref{fig:framework}.
% In the following we will present the details 


% implement three layers, which are user activity  embedding layer embedding layer, multi-perspective similarity learning layer and sequence based prediction layer. 
% The embedding layer takes the sequences of users and projects the them into a dense vector for each time point, which uses the hidden states as the outputs.
% The obtained dense features will be fed into the second layer that compute the similarity for time point. Finally, we apply an attention layer to output a score for determining the similarity.



\subsection{Methodology}
First, we present an overview of our proposed framework, \ourmeth, for friend suggestions, which exploits users' long-term and short-term information. 
Then we introduce the main components of \ourmeth  in detail: structured sequence embedding layer, multi-view similarity modeling layer, and similarity evolution layer. 



% We first present the general NCF framework, elaborating how to learn NCF with a probabilistic model that em- phasizes the binary property of implicit data. We then show that MF can be expressed and generalized under NCF. To explore DNNs for collaborative filtering, we then pro- pose an instantiation of NCF, using a multi-layer perceptron (MLP) to learn the user–item interaction function. Lastly, we present a new neural matrix factorization model, which ensembles MF and MLP under the NCF framework; it uni- fies the strengths of linearity of MF and non-linearity of MLP for modelling the user–item latent structures.




\subsubsection{General Framework}
In this paper, we propose a novel friend suggestion framework by ranking people in the candidate set after retrieval through a multi-stage deep structure. 
% %, underlining the time dependency and multiple perspectives of sequence data of online users. 
An overview of our proposed model is shown in Figure ~\ref{fig:framework}.
% In the following we will present the details 
% implement three layers, which are user activity  embedding layer embedding layer, multi-perspective similarity learning layer and sequence based prediction layer. 
The embedding layer takes user behavior sequences as input and projects them into a dense vector for each time point, which uses hidden states as output. 
Then the output embedding of each time slot is concatenated with the user's static profile vector, which can comprehensively capture user's long-term and short-term interests. 
Subsequently, the obtained dense features are fed into the second layer to obtain users' historical interests from multi-view viewpoints. 
Finally, we apply an evolutionary similarity layer to output a score to determine the similarity. 










% \subsubsection{User activity  embedding layer}
\subsubsection{ Structured sequence embedding layer.}
% \subsubsection{Gated Recurrent Unit embedding}
% \par
% in order to model the input sequences, we apply sequence-aware neural networks to
% The most distinctive characteristic of our setting is to take pair-wise sequences
\eat{
\textcolor{red}{Different from traditional e-commerce recommendations or news recommendations, in a large number of social apps and game apps, the user’s friendship behavior is sparse and random, which is not suitable for modeling user's friend interests via user's interaction sequence with strangers.
In these scenario, the user’s interaction with the app and activity in the app is very rich even if it has less relation with user's friend preference.
Thus, how to utilize these behavior to conduct friend recommendation is vital and difficult.}\todo{this part should not be here. the model section should tell what model looks like, as to the reason/motivation should be at somewhere else.}
}


Individual players constantly output a series of actions in the game, providing rich information to understand the players' state over time. 
The friend suggestion setup needs to understand the recent changes made by the user. 
We therefore start by modeling activity sequences which has directly or indirectly related to the user's friend application preference. 
First, we transform the user's activity sequences $S (x^{(1)}, x^{(2)}, ..., x^{(t)})$ into a dense representation via an embedding layer, where we take the most up-to-date  $t$ time steps from the user's records and pad the sequence with zeros if one does not have enough data. 
We know that Recurrent Neural Network (RNN) and its variants have the ability to capture inherent sequential dependency, hence we implement this style-based embedding layer to extract features preserving user characteristics. 
% For modeling the continuous behavior of user during the game, such as matches and battles.
We adopt Gated Recurrent Units (GRU)~\cite{chung2014empirical} here because it alleviates the vanishing gradient problem and does not yield more learnable parameters as in RNNs, which can be stated as follows,
% to capture the inherent sequential dependency and obtain the user embedding which can reflect the users' interests. 
% Compared with Recurrent Neural Network (RNN), GRU can alleviates the
% problem of vanishing gradient and does not bring more learnable parameters. 
% More specifically, GRU in our framework can be expressed as:
% \begin{align}
%     \mathbf{u^{(t)}} &= {\rm sigmoid}(g([\mathbf{X^{(t)}};\mathbf{H^{(t-1)}}] + b_u),
%     \notag
%     \\
%     \mathbf{r^{(t)}} &= {\rm sigmoid}(g([\mathbf{X^{(t)}};\mathbf{H^{(t-1)}}] + b_r),
%     \notag
%     \\
%     \mathbf{C^{t}} &= {\rm tanh}(g([\mathbf{X^{(t)}};\mathbf{r^{(t)}\cdot H^{(t-1)}}] + b_c),
%     \notag
%     \\
%     \mathbf{H}^{(t)} &= \mathbf{u}^{(t)} \odot \mathbf{H}^{(t-1)} + (1 - \mathbf{u}^{(t)}) \odot \mathbf{C}^{(t)},
%     \notag
% \end{align}
\begin{equation}
    \begin{cases}
\mathbf{u}^{(\mathbf{t})}= \sigma  \left(g\left(\left[\mathbf{X}^{(\mathbf{t})} ; \mathbf{H}^{(\mathbf{t}-\mathbf{1})}\right]+b_{u}\right)\right.\\
\mathbf{r}^{(\mathbf{t})}=\sigma \left(g\left(\left[\mathbf{X}^{(\mathbf{t})} ; \mathbf{H}^{(\mathbf{t}-\mathbf{1})}\right]+b_{r}\right)\right.\\
\mathbf{C}^{\mathbf{t}} =\tanh \left(g\left(\left[\mathbf{X}^{(\mathbf{t})} ; \mathbf{r}^{(\mathbf{t})} \cdot \mathbf{H}^{(\mathbf{t}-\mathbf{1})}\right]+b_{c}\right)\right.\\
\mathbf{H}^{(t)} =\mathbf{u}^{(t)} \odot \mathbf{H}^{(t-1)}+\left(1-\mathbf{u}^{(t)}\right) \odot \mathbf{C}^{(t)}
\end{cases}
\end{equation}
where $\mathbf{X}^{(t)}$ and  $\mathbf{H}^{(t)}$ represent the input and output at time step $t$; 
$\mathbf{X}^{(t)}$ represents the values of different behavior sequences at time $t$ and $\mathbf{X}^{(t)} \in $ $\mathbb{R}^{d \times 1}$, where $d$ is dimension of input features;
$g(\cdot)$ signifies the fully connected function; $\sigma $ denotes the sigmoid activation function; $ \odot$ is the Hadamard product operation. Besides,  $\mathbf{u}^{(\mathbf{t})}$ and $\mathbf{r}^{(\mathbf{t})}$ are the update gate  at $t$ step and reset gate at $t$ step, respectively.
\par
In this layer, each encoder unit extracts the feature vectors of an input sequence and projects the temporal dependency into a hidden representation. 
This means that at each time slot, each user has a unique representation vector that can reflect activity such as skill dynamics in the game.
%or patterns in the dating application. 



After obtaining the embedding for each time slot, we combine it with the long-term features of the players, i.e., profiles. 
The underlying assumption is that one intermediate action of a player may deviate from his/her normal patterns and mislead the similarity estimation process.  Meanwhile, the long-term information alone may not always reflect the player's current preferences. 
It is therefore necessary to combine these two together as an input for computing the similarity at each time step. 
For each user, the hidden state representation is $\mathbf{H^{(t)}}$ and the user's profile features is  $\mathbf{S^{(t)}}$, and the concatenation output is $\mathbf{e^{(t)}}$.


% As we mentioned earlier that users generate the long-term
% and short-term information simultaneously, therefore, it is important to integrate them together to produce an efficient representation for users.

% \textcolor{red}{These information makes different contributions to modeling user interests, and the two types of information have different interaction relationships at different historical moments.}
 %But these two have different properties from the time perspective. 
% Intuitively, these two types of information mutually influence each other.
% One intermediate action of a player may deviate from his/her normal pattern and mislead the estimation of similarity. Long-term information alone may not always reflect a player's current preference.

% Therefore, it is necessary to integrate long-term information with actions at each time. 



% \subsubsection{Dynamic blending layers}\\
% As we mentioned earlier that users generate the long-term
% and short-term information simultaneously, therefore, it is important to integrate them together to produce an efficient representation for users.
% % \textcolor{red}{These information makes different contributions to modeling user interests, and the two types of information have different interaction relationships at different historical moments.}
%  %But these two have different properties from the time perspective. 
% % Intuitively, these two types of information mutually influence each other.
% One intermediate action of a player may deviate from his/her normal pattern and mislead the estimation of similarity. Long-term information alone may not always reflect a player's current preference.
% Therefore, it is necessary to integrate long-term information with actions at each time. 

% \textcolor{blue}{As we mentioned earlier that users generate the long-term
% and short-term information simultaneously, therefore, it is important to integrate them together to produce an efficient representation for users.
% % \textcolor{red}{These information makes different contributions to modeling user interests, and the two types of information have different interaction relationships at different historical moments.}
%  %But these two have different properties from the time perspective. 
% % Intuitively, these two types of information mutually influence each other.
% One intermediate action of a player may deviate from his/her normal pattern and mislead the estimation of similarity. Long-term information alone may not always reflect a player's current preference.
% Therefore, it is necessary to integrate long-term information with actions at each time. 

% To act may amplify difference 
% Specifically, long-term information has influence on each action of a player, therefore, integrating such information into each time point toghther with 
% }

% therefore, we can assume there is underlying connections among these information, also called as the latent graph. 
% We aim to infer this graph and embed its structure information into users' data sequences.




\subsubsection{Multi-view similarity modeling layer}
From the previous step of our model, we obtain a time-aware representation of the players. 
We now introduce a new simple yet effective method for computing the similarity between users. 
% through multiple perspectives.
% Given that we intend to quantize the similarity between users, we introduce a new simple but effective method to compute this through multiple perspectives.
% We now present a generalization solution for measuring the similarity between the embedding features.  
Often, recommendation systems use dot product to get the similarity between input embedding pairs $(\mathbf{e_i}, \mathbf{e_j})$, denoting $ \mathbf{e_i^T} \mathbf{e_j}$. 
With simply linear algebra knowledge, we know that this score function can be formulated as a bilinear form of $\mathbf{e_i^T I e_j}$, where $\mathbf{I}$ is an identity matrix. However, this undermines the importance of the similarity function since the similarity measure and embedding should be mutually enforced to achieve recommendation success. 
This abandons the discriminative power of the similarity function by using the identity matrix, making the prediction models fully dependent on the embedding. 
To overcome this limit, we choose to learn  a parametric similarity subspace, $\mathbf{W}\in\mathbb{R}^{m \times m}$, to better fit the data, resulting in a general similarity measurement as $M(\mathbf{e_i,e_j}) =\mathbf{e_i^T W e_j}$.  
Also, learning a single similarity matrix may not be able to fully capture the relations between input feature-pair embeddings. 
Inspired by ensemble learning theory, we aim to learn a group similarity function to determine similarity collectively. More specifically, we can formulate ensemble similarity learning as: 
\begin{equation}
 M(\mathbf{e_i,e_j}) =\sum_k\mathbf{e_i^TW^ke_j} 
 %= \sum_k W^k\otimes \left ( e_i^Te_j \right )=\sum_k\sum_{pq}W_{pq}^ke_{ip}e_{jq}
\end{equation}
where $W^k$ denotes the $k$th similarity matrix. To implement this, we can further rewrite this bilinear into a linear format like the following:
\begin{equation}
 M(\mathbf{e_i,e_j}) =\sum_k\mathbf{e_i^TW^ke_j} = \sum_k \mathbf{W^k}\otimes \left (\mathbf{e_i^Te_j} \right )=\sum_k\sum_{pq}\mathbf{W_{pq}^ke_{ip}e_{jq}}
\end{equation}
By vectorization, we have $ \mathbf{z} = \left ( \mathbf{e_{i1}}*\mathbf{e_{j1}},...,\mathbf{e_{im}}*\mathbf{e_{jm}} \right )^T$ and $\mathbf{s^k} = \left ( \mathbf{W_{11}^k},\mathbf{W_{21}^k}...,\mathbf{W_{mm}^k} \right )^T$, and reformulate the similarity measurement as follows,
\begin{equation}
     M(\mathbf{e_i,e_j}) =\sum_k\mathbf{e_i^TW^ke_j} = \left [\mathbf{s^1},\mathbf{s^2},...,\mathbf{s^k} \right ]^T\mathbf{z} % =S^Tz
\end{equation}
This can be implemented as a standard MLP network having
\begin{equation}
    \begin{aligned}
    % &\mathbf{z}_{1} = [\mathbf{x},\mathbf{y}]\\
    % &....\\
\mathbf{g} &=u\left(\mathbf{S}^{T}  {\mathbf{z}}+{b}\right)  \\
% &\hat{y} &=\sigma\left(\mathbf{h}^{T} \phi_{L}\left({z}_{L-1}\right)\right)
\end{aligned}
\end{equation}
where $b$ is the bias term and $\mathbf{S} = \left [\mathbf{s^1},\mathbf{s^2},...,\mathbf{s^k} \right ]$. Here, $u()$ is activation function, and we use ReLU to promote sparsity in outputs.


% \todo{we can decide whether or not add this bias term of mlp, may be we should?}
% To fully exploit the information in features, we also consider a naive combination of features from both users, denoted as $\mathbf{b}_{L} =V_L^T[e_i; e_j]$ 

% we propose a sequential loss function for this purpose, which is written as 
% \begin{equation}
%     \begin{aligned}
%         l(\mathbf{u}_i, y_{i})= \lambda p\left(y_{i} \mid \mathbf{u}_{i}\right)+(1-\lambda)  q\left(z_{i} \mid z_{i-k}, \cdots, z_{i-1}\right)
%     \end{aligned}
% \end{equation}


% \subsubsection{Similarity evolution sequence}


% \subsection{Sequence based prediction }

\subsubsection{Similarity evolution modeling layer.}
% \textcolor{red}{After we obtain the similarity sequence via multi-view similarity modeling layer, we aim to learn a user-pairs similarity pattern from this sequences.}
So far we have obtained the similarity embedding at each time point for a given pair users. 
The goal of this layer is to produce user-user pair similarity based on the output from the multi-view similarity modeling layer. 
As stated before, the similarity between a pair of users will evolve over time. 
For example, online game players will change their strategy of adding strangers according to their own level changes, and naturally the similarity between users will evolve over time.  
The historical similarities will have different relevance effects on the current time slot, therefore the problem now translates into capturing this underlying relevance. 
% In addition, different users tend to add friends with different level distributions, and the similarity sequence mined from user behavior will have an impact on the application preferences at the current moment.
We know that the attention mechanism has been proven to be most effective of capturing relevant information, therefore, we employ this to learn the underlying similarity evolution automatically.
Specifically, we implement our similarity evolution modeling layer by leveraging TransFormer's self-attention module, in which each time point is used as a word and whole group as a sentence. 
For each word, we can obtain the attention score as following,
 \begin{align}
    \mathrm{Att}(\mathbf{Q}, \mathbf{K}, \mathbf{V}) = \mathrm{SoftMax}(\frac{\mathbf{Q}\mathbf{K}^\top}{\sqrt{d_k}})\mathbf{V},
\end{align}
where $\mathbf{Q}$, $\mathbf{K}$ and $\mathbf{V}$  $\in \mathbb{R}^{T\times d_k}$ represent Query, Key and Value vectors, respectively.
% where $\mathbf{Q}$, $\mathbf{K}$ $\in \mathbb{R}^{T\times d_k}$.
Here, $d_k$ represents the embedding dimension of the item. 
Besides, by following~\cite{2017Attention}, we add multi-head attention mechanism
to capture the correlation in different representation sub-spaces. 
 \begin{align}
    \mathrm{MultiAtt}(\mathbf{E}) &= \mathrm{Concat}(head_1, head_2, ..., head_n)\mathbf{W^H},
    \notag
    \\
    head_i &= \mathrm{Att}(\mathbf{E\Theta^Q}, \mathbf{E\Theta^K}, \mathbf{E\Theta^V},)
\end{align}
where $\mathbf{E}$ is the input embedding of each time point, and $\mathbf{\Theta^Q}$, $\mathbf{\Theta^K}$, $\mathbf{\Theta^V}$ are all projection matrices.
\par
Note that the self-attention layer neglects the relative position in the sequence since it treats different positions equally while obtaining the attention score.  
In order to capture the relative position of $\mathbf{E_t[i,:]}$ in the entire sequence,
we employ the position encoding as in~\cite{2017Attention} to represent the sequence relationship while considering the locations of words. Specifically, we add position encoding vector with input embedding as the input of self-attention.
 \begin{align}
    \mathbf{E^{'}_{t}[i,:]}=\mathbf{E_t[i,:]} + \mathbf{p_t},
\end{align}
where $\mathbf{p_t}$ is defined as:
 \begin{align}
    \mathbf{p_t} = \left\{
\begin{aligned}
sin(t/10000^{2i/d_{model}}), t=0,2,4.. \\
cos(t/10000^{2i/d_{model}}), t=1,3,5..
\end{aligned}
\right.
\end{align}
In this way, instead of directly utilize the output of multi-view similarity modeling layer, we use the one with positional encoding as input for the self-attention layer. After the multi-head attention layer extracting the relations between similarity sequence, we transmit the output to a point-wise feed-forward neural network layer to generate the score of user-pairs.

\subsubsection{Loss function.}
To predict whether a user-pair will establish a friend-request connection, we model it as a binary classification task, and use sigmoid function as the output unit. 
In this work, we use the cross-entropy loss to train our model:
\begin{equation}
    \mathcal{L}(\theta)=-\frac{1}{N}\sum_{(x,y)\in \mathcal{D}} (ylogp(\theta) + (1-y)log(1-p(\theta))
\end{equation}
where \mathcal{D} denotes all the training samples and $y \in \{0,1\}$ is the groundtruth whether user A has applied user B or not, $\p(\theta)$ is the output of our framework which represents the prediction probability.

% Considering the matter of positions of each word, we utilize position encoding as in~\cite{2017Attention} to represent the sequence relationship.

% \textbf{Output or classifier:}
% \todo{we need this section, right? }
% \textcolor{red}{In this section, it is only a linear projection layer with a sigmoid activation function, so we just mention it is enough?}



% \begin{table*}
% % \footnotesize
% \scriptsize
% \centering
% \begin{tabular}{|l|llllllll|llllllll|}
% \arrayrulecolor{black}\hline
% Dataset &      &      &      &  D1     &       &       &       &        &      &      &      &     &     D2    &       &       &         \\ 
% \hline
% Metric  & N@10 & N@20 & N@50 & N@100 & HR@10 & HR@20 & HR@50 & HR@100 & N@10 & N@20 & N@50 & N@100 & HR@10 & HR@20 & HR@50 & HR@100  \\ 
% \hline
% MLP     &  0.0950    & 0.1051     &   0.1158   &  0.1237     &       0.1469 &0.1871       &    0.2413   &  0.2903      &      &      &      &       &       &       &       &         \\
% GRU     & \textbf{0.1032}    &  0.1126    &   0.1232   &  0.1301     &       0.1520 &  0.1895     &  0.2429     &   0.2850     &      &      &      &       &       &       &       &         \\
% DSEN-LSTM   &  0.1012    &    0.1112  & \textbf{0.1241}     & 0.1304      &     \textbf{0.1561}  &    0.1955   &0.2602       &  0.2991      &      &      &      &       &       &       &       &         \\
% DSEN-ATT   &  0.1011    &   \textbf{0.1114}  &  \textbf{0.1241}   &    \textbf{0.1306}   &      0.1554 &    \textbf{0.1962}   &   \textbf{0.2604}    &  \textbf{0.3005 }     &      &      &      &       &       &       &       &         \\ 
% \hline
% Gains   &   -1.9\%   &  6.0\%    &   7.1\%   &    5.5\%   &    6.2\%   &   4.7\%    &    7.9\%   &      5.4\%  &      &      &      &       &       &       &       &         \\
% \hline
% \end{tabular}
%  \caption{ \footnotesize
% Friend suggestion comparison of the competing techniques on two large datasets: section $1$ and section $2$. }
%     \label{tbl:COMPARSION}% \vsa\vsb

% \end{table*}

% \begin{table*}
% % \footnotesize
% \scriptsize
% \centering
% \begin{tabular}{|l|llllllll|llllllll|}
% \arrayrulecolor{black}\hline
% Dataset &      &      &      &  D1     &       &       &       &        &      &      &      &     &     D2    &       &       &         \\ 
% \hline
% Metric  & N@10 & N@20 & N@50 & N@100 & HR@10 & HR@20 & HR@50 & HR@100 & N@10 & N@20 & N@50 & N@100 & HR@10 & HR@20 & HR@50 & HR@100  \\ 
% \hline
% MLP     &  0.0334    & 0.0429     &   0.0589   &  0.0711     &       0.0688 & 0.1063       &    0.1877   &  0.2629      &      &      &      &       &       &       &       &         \\
% GRU     & 0.0987    &  0.1111    &   0.1249  &  0.1333     &       0.1547 &  0.2039     &  0.2733     &   0.3252     &      &      &      &       &       &       &       &         \\
% DSEN-LSTM   &  0.1020    &    0.1138  & 0.1281    & 0.1365      &    0.1619  &    0.2093   &0.2805       &  0.3325      &      &      &      &       &       &       &       &         \\
% DSEN-ATT   & \textbf{0.1071}    &   \textbf{0.1207}  &  \textbf{0.1359}   &    \textbf{0.1448}   &       \textbf{0.1680} &    \textbf{0.2222}   &   \textbf{0.2986}    &  \textbf{0.3532 }     &      &      &      &       &       &       &       &         \\ 
% \hline
% Gains   &   +\%   &  +\%    &   +\%   &    +\%   &   +\%   &  +\%    &    +\%   &      +\%  &      &      &      &       &       &       &       &         \\
% \hline
% \end{tabular}
%  \caption{ \footnotesize
% Friend suggestion comparison of the competing techniques on two large datasets: section $1$ and section $2$. }
%     \label{tbl:COMPARSION}% \vsa\vsb

% \end{table*}



%+++++++++++++
%+++++++++++++
%+++++++++++++
%+++++++++++++


\begin{table*} [t]
\setlength{\abovecaptionskip}{0.3cm}
\centering
 \small
\caption{Friend suggestion comparison of the competing techniques on two large datasets}
\begin{tabular}{llrrrrrrrrr}
%\hline
%\toprule[1pt]
\toprule
\multirow{2}{*}{Dataset} & \multirow{2}{*}{models} & \multicolumn{2}{c}{K=10}         & \multicolumn{2}{c}{K=20}       & \multicolumn{2}{c}{K=50}    & \multicolumn{2}{c}{K=100}                       \\ \cline{3-10}
                         &                         & HIT@K           & NDCG@K                   & HIT@K           & NDCG@K                 & HIT@K           & NDCG@K         & HIT@K           & NDCG@K              \\ %\hline
\midrule
                        % & HA   & 4.16 & 7.80 &13.0\% & 4.16 & 7.80 &13.0\% & 4.16 & 7.80 &13.0\%
                        % \\
                         & MLP   &  0.0688    & 0.0334     &   0.1063   &  0.0429     &       0.1877 & 0.0589       &    0.2627   &  0.0711            \\
                         
                         & GRU                 &  0.1547    &  0.0987    &   0.2039  &  0.1111     &       0.2733 &  0.1249     &  0.3252     &   0.1333     \\
                   
                         & self-Attention    &   0.1662     &   0.1050   &   0.2189  &  0.1183     &  0.2897    &  0.1324     &    0.3459   &  0.1415     \\
   Section-1  
                       & \textbf{DSEN}          & \textbf{  0.1680}    &   \textbf{0.1071}  &  \textbf{0.2222}   &    \textbf{0.1207}   &       \textbf{0.2986} &    \textbf{0.1359}   &   \textbf{0.3532}    &  \textbf{0.1448}      \\

\midrule
                        % & HA & 2.88 & 5.59 & 6.8\% & 2.88 & 5.59 & 6.8\% & 2.88 & 5.59 & 6.8\%
                        % \\
                         & MLP                   &   0.1780       &        0.1059         &   0.2358       &   0.1204              &         0.3149 &     0.1362 & 0.3773 & 0.1463        \\
                         & GRU                 &     0.1784     & 0.1109                 &      0.2328     &    0.1246               &       0.3142  &       0.1407 & 0.3728 & 0.1502           \\
                         & self-Attention         &    0.1881     &    0.1130              &  0.2464     &    0.1278             & 0.3312         &          0.1446 & 0.3888 & 0.1540     \\
   Section-2  
                       & \textbf{DSEN}              &   \textbf{0.1914 }      &     \textbf{0.1167   }    &     \textbf{0.2499 }      &   \textbf{0.1315 }                &  \textbf{0.3421 }     &      \textbf{0.1498}  & \textbf{0.4050}  & \textbf{0.1600 }            \\
                       
\midrule
                        % & HA & 2.88 & 5.59 & 6.8\% & 2.88 & 5.59 & 6.8\% & 2.88 & 5.59 & 6.8\%
                        % \\
                         & MLP   &     0.1796    &   0.1108             & 0.2334        &   0.1244              & 0.3062  & 0.1389   & 0.3615 &  0.1479       \\
                         & GRU                 &     0.1840     & 0.1173                 &      0. 2330    &    0.1296              &       0.3069  &       0.1444 & 0.3587 & 0.1528           \\
                         & self-Attention         &    0.     &    0.              &  0.     &    0.             & 0.         &          0. & 0. & 0.     \\
   Section-3  
                       & \textbf{DSEN}              &   \textbf{0.1846 }      &     \textbf{0.1159}    &     \textbf{0.2363 }      &   \textbf{0.1289 }                &  \textbf{0.3117 }     &      \textbf{0.1439}  & \textbf{0.3679}  & \textbf{0.1531}            \\
\bottomrule
\end{tabular}\label{tbl:COMPARSION}
\label{table_2}
\vspace{-2mm}
\end{table*}







==> tex/0_timeline.tex <==
\section{time line}



0626--0703 

完成模型代码；

完成部分论文文字：introduction/relate work 

准备数据：公司数据，考虑公共数据集


---
0704--0717

试验测验codm：
第一部分：codm小数据
第二部分：offline codm测试 （周二/三出几个结果，包括对比的模型）
第三部分：online  codm（如果时间来得及）（inference spark）
 
ablation实验怎么做 (暂定去掉mltiview mlp那一层)


 
初稿：intro+related+model

---
0718--0731
实验：
第一部分：online 实验
第二部分：要么新游戏，要么公共改造
第三部分：ablation study

---
0801-089 
写作+完善实验
注册wsdm





